Hypothesis Transfer Learning with Surrogate Classification Losses: Generalization Bounds through Algorithmic Stability

Hypothesis transfer learning (HTL) contrasts domain adaptation by allowing for a previous task leverage, named the source, into a new one, the target, without requiring access to the source data. Indeed, HTL relies only on a hypothesis learnt from such source data, relieving the hurdle of expansive data storage and providing great practical benefits. Hence, HTL is highly beneficial for real-world applications relying on big data. The analysis of such a method from a theoretical perspective faces multiple challenges, particularly in classification tasks. This paper deals with this problem by studying the learning theory of HTL through algorithmic stability, an attractive theoretical framework for machine learning algorithms analysis. In particular, we are interested in the statistical behaviour of the regularized empirical risk minimizers in the case of binary classification. Our stability analysis provides learning guarantees under mild assumptions. Consequently, we derive several complexity-free generalization bounds for essential statistical quantities like the training error, the excess risk and cross-validation estimates. These refined bounds allow understanding the benefits of transfer learning and comparing the behaviour of standard losses in different scenarios, leading to valuable insights for practitioners.

==> conclusion.tex <==
Sanity check bounds are difficult to improve upon without further assumptions regarding  algorithm stability,
\eg loss stability as introduced in \cite{kumar2013near}, where the variance of the K-fold \CV is shown to be $K$-times smaller than that of the empirical risk.
A lead for further research  would be to consider such wider classes of
algorithms, for which various stability
hypotheses replace advantageously the assumption of finite \VC
dimension % , allowing among others to analyze %obtain finite sample guarantees
% %regarding
% \CV estimates of the risk
(see \eg
\cite{kearns1999algorithmic,BousquetElisseeff-2000,bousquet2002stability}). % stability notions allow  in some cases significant improvement over sanity-check bounds, which consitutes a major lead for further research in the rare class setting considered here. 

% It goes
% without saying: extending our results to
% other or more general \EVT-related problems
% and algorithms will be subject of further research.  In particular
Another promising avenue would be to consider unsupervised problems  which are the main field of application for 
\EVT. Also, while  we limit ourselves to risk estimation, we hope that our work can pave  the way towards a theoretical understanding of \CV-based  hyper-parameter selection in \EVT algorithms. % where such parameters are ubiquitous. 

Finally, even though our work is motivated by the \EVT framework, no regular variation assumption is needed for our results to hold regarding \CV risk estimates, and the precise definition of the rare class $\mathbb{A}$ is unimportant, only the small probability $\alpha$ is. Thus we believe that our results and techniques of proof could
  serve in other \ML contexts involving a rare class, such as imbalanced multi-class classification where the learner  must distinguish between several  minority classes. 

  %%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_crossval.tex"
%%% End:


==> framework.tex <==
In this paper, we analyse hypothesis transfer learning by mean of regularised empirical risk minimization (\textrm{RERM}). Such a general family of \HTL algorithms  includes in particular Regularized Least Squares (\textrm{RLS}) with biased regularization \cite{orabona2009,kuzborskij2013,kuzborskij2017fast}. Formally we consider the following algorithm,
\begin{equation}\label{def:algo-transfer}
    \alg= f(\DD_T)+ h_S
\end{equation}
where $f$ is the  obtained via the minimization problem:
\begin{align}\label{def:algo-training-transfer}
f&= \argmin_{h \in \mathcal{H}_T}\frac{1}{n}\sum_{i=1}^n\phi\left(\left(h\left(X_i\right)+h_S\left(X_i\right)\right)Y_i\right)+\lambda_n\lVert h\rVert_k^2\nonumber\\
&=\argmin_{h \in \mathcal{H}_T}\ER(h+h_S)+\lambda_n\lVert h\rVert_k^2.
\end{align}
The family of classifiers $\mathcal{H}_T$  is a reproducing kernel Hilbert space (\textsc{RKHS}) endowed with a kernel $k$ , a scalar product $\langle \cdot,\cdot\rangle$ and a norm $\lVert\cdot\rVert_k$. In the following we will assume that the kernel $k$ is bounded by $\kappa$ \ie
$$\forall x \in \mathcal{X}_T\;,\; k(x,x)\leq \kappa.$$
\begin{remark}[link with RLS]\label{remark:rls-link}
	By choosing $k$ as the linear kernel \ie $k(x_1,x_2)=x_1^\top x_2$ and $\phi(x)=\left(1-x\right)^2$ Algorithm \ref{def:algo-transfer} is equivalent to,
	$$\alg=f+h_S$$
	with
 \begin{align*}
    f&=\argmin_{u \in \rset^d}\frac{1}{n}\sum_{1}^{n}\left(u^\top X_iY_i +h_S(X_i)Y_i-1\right)^2+\lambda_n\lVert g\rVert_k^2 \\
    &=\argmin_{u \in \rset^d}\frac{1}{n}\sum_{1}^{n}\left(u^\top X_i +h_S(X_i)-Y_i\right)^2+\lambda_n\lVert g\rVert_k^2.
 \end{align*}
	
   \ag{Discussion prochain réunion : plus de details pour le dernier passe ou pas besoin?}Therefore, \textsc{RLS} with biased regularization   is a special case of the proposed algorithm.
\end{remark}

\begin{discussion*}[Difference with the regression case]
\textsc{RERM} for regression is equivalent to fitting a predictor on the residuals $Y_i-h_S(X_i)$. However, in the classification case, if we follow the standard approach that $h_S: \mathcal{X}\mapsto \mathcal{Y}=\{-1,1\}$ is a binary classifier \cite{kuzborskij2013,cortes2015adaptation,du2017hypothesis} .  the latter residuals are either $1$ or $0$  and for many losses this won't provide enough information to improve the training. To see this, take the example of the logistic loss and notice that $\phi(1)=\log(1+e^{-1})$ or $\phi(-1)=\log(1+e^1)$. Therefore, in the best case scenario, $\loss(h_S,O)=\log(1+e^{-1})$  which is far from the minimum (0).\\
To tackle this problem, we suggest to take the score learned on the source which is more informative especially when the loss function used to train the algorithm on the source have the same minimum as the loss used to train on the target. \\
Note that, one can also think of transforming the score, for example if $\phi$ 
 is the logistic loss $\phi(x)=\log(1+e^{-x})$ and $h_S\in ]-1,1[$ we can use an increasing transformation function to an interval $]-C,C[$ with $C>>1$ in order to adapt to the target loss which is nearly 0 for large values $x$ . 
 
 % Then, using the target dataset $\DD_T$, we try to \textbf{adapt}  the hypothesis score $h_S$ by adding another score $f$ (cf. Equation \ref{def:algo-training-transfer}) that depends directly on the  performance of $h_S$ \big($\ER[h_S]$\big). More details will be provided in the rest of this section. 
\end{discussion*}
In order to analyse the stability of Algorithm \ref{def:algo-transfer} we start by showing that the solution of the problem \ref{def:algo-training-transfer} lies in the sphere $\left\{g\in\mathcal{G}\; \big \lvert\; \lVert g \rVert_\infty \leq  \hat r_\lambda \right\}$ with
$$\hat r_\lambda= \sqrt{\alpha\left(\ER^{\backslash i}\left[h_S\right]+\frac{\norm{\phi\circ g^\prime}_\infty}{n}\right)}, $$
and $\alpha=\frac{\kappa}{\lambda}$. Besides, by using the optimality condition of problem \ref{def:algo-training-transfer} and the Bregman divergence  we deduce that the stability parameter $\beta_n$ verifies (up to a constant factor)
\begin{align*}
\beta_n&\leq  \frac{1}{n}\EE\left[\phi'\left(\left(h_S(X_i)+f(X_i)\right)Y_i\right)^2\right]\\
&\leq \frac{1}{n}\EE\left[\sup_{\abs{y}\leq \hat r_\lambda} \phi'(h_S(X)Y+y)^2 \right] 
\end{align*}
and for many surrogate losses the right hand term is bounded by $\Psi\left(\risk\left[h_S\right]\right)/\left(\lambda n\right)$ for some decreasing function $\Psi$ verifying $\Psi(0)=0$ . Formally, we will show that all the losses in the Introduction verifies the following Property  .
\begin{property}\label{property:derivative-expectation}
The function $\phi$ is decreasing, differentiable, convex and verifies the following inequality
\begin{align*}
	\EE\left[\sup_{\abs{y}\leq \hat r_\lambda} \left|\phi'(h_S(X')Y'+y)\phi'(h_S(X)Y+y)\right|\right]&\\
	&\hspace{-20mm}\leq \Psi\left(\risk\left[h_S\right]\right)+\mathcal{O}\left(\ffrac{1}{n}\right),
\end{align*}
where $Z=(X,Y)$, $Z'=(X',Y')$ are two samples drawn from $P_T$ indepedent of $\DD^{\backslash i}$  and $\Psi$ is a decreasing function  verifying $\Psi(0)=0$.
\end{property}
% The function $\phi$ is decreasing convex and verifies the following twin inequalities for all $i\in [n]$
% \begin{equation*}
% 	\EE\left[\sup_{\abs{y}\leq \hat r_\lambda} \phi'(h_S(X)Y+y)^2\right]\leq \Psi_1\left(\risk\left[h_S\right]\right)+\mathcal{O}\left(\ffrac{1}{n}\right),
% \end{equation*}
% \begin{align*}
% 	\EE\left[\sup_{\abs{y}\leq \hat r_\lambda} \left|\phi'(h_S(X')Y'+y)\phi'(h_S(X)Y+y)\right|\right]&\\
% 	&\hspace{-20mm}\leq \Psi_2\left(\risk\left[h_S\right]\right)+\mathcal{O}\left(\ffrac{1}{n}\right),
% \end{align*}

%The next property if verified by some exponential like loss functions .
%\begin{property}{Mult} \label{property:mult}
%The function $\phi$ is decreasing convex and verifies for all $B>0$ and $\abs{y}\leq B$ 
%\begin{equation}
%\left|\phi'(x+y)\right|\leq \Psi_1\left(\phi(x)\right)\Psi_2(B).
%\end{equation}
%
%Where $\Psi_2$ is a non negative continuous function and $\Psi_1$ is a non decreasing concave function on $$\mathcal{S}_{B}=\left\{x \in \rset \mid \Psi_1\left(\phi(x)\right)\Psi_2(B)\leq \phi'_\infty \right\},$$
%and verifying $\Psi_1(0)=0$.
%\end{property}

\begin{discussion*}[comparison with existing assumptions]
In the \HTL literature they generally assume that the loss function verifies a smoothness condition, for example in \citet{cortes2015adaptation} they suppose that $\loss$ is Lipschitz, which doesn't hold for the MSE when $\mathcal{X}_T$ is unbounded.  In \citet{kuzborskij2017fast} they assume that the derivative is Lipschitz which is not the case for the exponential. Furthermore, even if the loss verifies this smoothness assumption the constants in the latter works depends heavily on the smoothness parameter and it would yield vacuous bounds in many practical situation. For example, the softplus function $\psi_s(x)=s\log(1+e^{\frac{1-x}{s}})$  with small values of $s$ serves as an approximation of the hinge loss ($\max(0,1-x)$). Thus the user picks generally a value of $s\ll 1$. Therefore,  the Liptchiz constant of the derivative $1/s$ verifies $1/s \gg 1$ and the bounds from \cite{kuzborskij2017fast} becomes vacuous. Another common assumption in the \HTL literature is the boundness of the loss $\loss(\alg,O)$   which is not necessarily verified for \textsc{RERM} when $\lambda_n\to 0$. The case $\lambda_n\to 0$ is indeed a key setting  since \textsc{RERM} are consistent with such a choice of $\lambda_n$ (see \eg \citet{Zhang2004,wibisono2009sufficient,kuzborskij2017fast}).\\
To our best knowledge, the vast majority of existing theoretical results from the \HTL literature have similar assumptions to those discussed above.  However, in this work our assumption is flexible : We don't require any precise smoothness property but we only require a majorant of the derivative which will make the analysis more flexible and more \textbf{suited } for the usual classification losses. \\
To understand the  intuition behind Property \ref{property:derivative-expectation} notice that, when $\risk[h_S]\to 0$, $h_s$ approaches the minimum and $\phi'(h_s)$ approaches 0. Thus, the function $\Psi$ dictates the rate of convergence of the derivative to $0$ when $h_s$ approches the optimal point \ie $\EE[\phi'\circ h_s]=\mathcal{O}\left(\Psi\circ\phi(h_S)\right)$ . 
\end{discussion*}
In the next Lemma we show that many loss functions verify the latter Assumption.
%On the other hand the function $\Psi_2$ controls the deviations of $\phi'(z)$ when $z$ is varying inThe next property if verified by some exponential like loss functions .
%\begin{property}{Mult} \label{property:mult}
%	The function $\phi$ is decreasing convex and verifies for all $B>0$ and $\abs{y}\leq B$ 
%	\begin{equation}
%	\left|\phi'(x+y)\right|\leq \Psi_1\left(\phi(x)\right)\Psi_2(B).
%	\end{equation}
%	
%	Where $\Psi_2$ is a non negative continuous function and $\Psi_1$ is a non decreasing concave function on $$\mathcal{S}_{B}=\left\{x \in \rset \mid \Psi_1\left(\phi(x)\right)\Psi_2(B)\leq \phi'_\infty \right\},$$
%	and verifying $\Psi_1(0)=0$.
%\end{property}
%a sphere around $x$. In the following lemma we show that this assumption is verified for many known losses

\begin{lemma}\label{lemma:loss-property}
The exponential, logistic, squared hinge , \MSE and softplus losses verifies Property \ref{property:derivative-expectation}. The corresponding function $\Psi$  are given by Table \ref{table:property-hypothesis}.
\end{lemma}
\begin{proof}
	The proof is  deferred to the appendix.
\end{proof}
\begin{table}
	\begin{center}
		\begin{tabular}{lccr}
			\hline
			loss  & $\Psi(x)$  \\[0.2cm] 
			\hline\\[-0.2cm]
                
		   exponential loss & $x^2e^{2\alpha x}$ \\ [0.2cm]
		   squared hinge & $8x(\alpha+1)$  \\ [0.2cm]
	       MSE  & $8x(\alpha+1)$  \\[0.2cm]
             
			logistic loss  &
			 $\ffrac{(e^{\sqrt{x}}-1)^2}{e^{-2\norm{h_S}_\infty}+e^{-2\sqrt{\alpha x}}}$ \\[0.2cm]
            softplus  & $\ffrac{(e^{\sqrt{x/s}}-1)^2}{e^{-2\norm{h_S}_\infty}+e^{-2\sqrt{\alpha x}}}$  \\[0.2cm]
			\hline
		\end{tabular}
	
		
	\end{center}
		\caption{deviations parameter for multiple losses}
            \label{table:property-hypothesis}
		% \label{table:loss-properties}
\end{table}
% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{lcccr}
% 			\hline
% 			loss  &  $\Psi_2(x)$ \\ 
% 			\hline
% 			logistic loss   & $(\exp\left(\sqrt{x}\right)-1)^2e^{2\alpha x}$ \\ 
% 			 softplus   & $(\exp\left(\sqrt{x/s}\right)-1)^2e^{2\alpha x}$   \\
% 			exponential loss & $x^2e^{2\alpha x}$\\ 
% 			squared hinge & $8x(\alpha+1)$ \\ 
% 			MSE   & $8x(\alpha+1)$ \\
% 			\hline
% 		\end{tabular}
	
		
% 	\end{center}
% 		\caption{deviations parameter for multiple losses}
% 		\label{table:loss-properties}
% \end{table}

% \subsection{The hinge loss}

% In order to cover the case of the hinge loss we will suppose that $\norm{g'}_\infty <1$. This assumption is indeed verified in many applications. For instance, if the source learning task is a binary classification problem where the classes $+1$ and $-1$ have a continuous densities $f_+,f_->0$ over $\mathbb{R}^d$. Then, if  $g'(x)\approx \frac{f_+}{f_++f_-} $ is a probability estimate, it is very likely to verify $\norm{g'}_\infty < 1$.

% \begin{lemma}\label{lemma:hinge-case}

% \end{lemma}

==> intermediate-mainpaper.tex <==
In this section we gather the main intermediate results involved in the proofs of our main results theorems~\ref{theo:main-sanity-rare} and~\ref{theo:main-sanity-rare-lpo}, which are of interest in their own.
% \todo{choose and insert key results here (lemmas A1, A2, corollaire A1 (?)}

A key tool to our proofs is  a Bernstein-type inequality relative to the deviation of a generic random variable $Z=f(O_1,\ldots,O_n)$ from its mean (\cite{McDiarmid98conc}) that we recall in the supplement for convenience (Proposition~\ref{"Bernstein-extension"}). The control of the deviations involves both a maximum deviation term and a variance term.   We leverage this result to control the deviations of the  pseudo-empirical risk $\tilde \risk_\alpha$ defined in ~(\ref{def:tilde-rcv}) averaged over the $K$ validation sets $V_{1:K}$. These deviations are embodied by the random variable $Z$ defined in Lemma~\ref{"RCV-supp"}, Equation~(\ref{def:Z-CV}), which is a key quantity when analysing the deviations of any \CV risk estimate as revealed by an inspection of the proofs in the supplement.  Controlling the deviations of $Z$ is the main purpose of this section.


%from  McDiarmid (see \ref{"Bernstein-extension"}) yields  the following lemma:

\begin{lemma}
	\label{"RCV-supp"}
Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables, and $V_1,V_2,\dots V_K$ a sequence of masks that verifies Assumption~\ref{assum:mask-property} with size $n_V$.\,Moreover,\,suppose that assumptions~\ref{assum:hypo-class} and~\ref{assum:cost-func} regarding the class $\mathcal{G}$ and $c$ hold. Define 
\begin{equation}\label{def:Z-CV}
Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,V_{j})-\mathcal{R}_\alpha(g) \rvert,
\end{equation}

where $\Tilde{\mathcal{R}}_{\alpha}$ is defined by Equation~\ref{def:tilde-rcv}.\,Then the random variable $Z$  satisfies the Bernstein-type inequality	
\[P\left(Z - E(Z) \geq t  \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).\]	
\end{lemma}


\begin{proof}
 The reader is referred to Appendix~\ref{"lemma-RCV-supp-proof"}.	
\end{proof}

To obtain a genuine probability bound on $Z$ \emph{via} the latter lemma, one also needs to control the term $E(Z)$. This is the purpose of the next lemma, the spirit of which is similar to Lemma 14 in~\cite{goix15}. The main difference \wrt to the latter reference is that we handle any bounded cost function (not only the Hamming loss), using a bound for Rademacher averages from~\cite{gine2001consistency} which applies in this broader setting.
\begin{lemma}
	\label{"RCV-expectation"}
        % For any subsample $S\subset \{1,\ldots, n\}$ of size $n_S$ define
	% \[
	% Z'=\sup_{g \in \mathcal{G}} \bigg|\Tilde{\mathcal{R}}_{\alpha}(g,S)-\mathcal{R}(g)\bigg|.
	% \]
	% Then we have
	% \[
	% \EE(Z') \leq B(n_S,\alpha),
	% \]
        In the setting of Lemma~\ref{"RCV-supp"}, $Z$ satisfies %we have
        \[
	\EE(Z) \leq   \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n_V}}.
	\]
%	where we define for a subsample size  $n_S\ge 0$, 
%\begin{equation}\label{"V-n-def"}
%%  {\color{red} + \frac{M_1  \vapnikG}{\alpha n_S}},
%\end{equation}  
where $M>0$ is a universal constant. % some constant $M>0$.
\end{lemma}

\begin{proof}	
	See Appendix~\ref{"proof-RCv-expectation"}
\end{proof}

The following probability upper bound for $Z$ follows immediately by combining Lemma~\ref{"RCV-supp"} and Lemma~\ref{"RCV-expectation"}. % the following corollary. 
\begin{corollary}
	\label{"RCV-sup-control"}
        In the setting of Lemma~\ref{"RCV-supp"}, 
	% Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables and $V_1,V_2,\dots V_K$ a sequence of masks satisfying assumption \ref{assum:mask-property}.  In addition suppose that assumption \ref{assum:hypo-class} and \ref{assum:cost-func} hold. Then
        we have
	\[P\left(Z - \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n_V}}\geq t \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right),\]
	where $Z$ is defined in \eqref{def:Z-CV}.
\end{corollary}
% \begin{myproof}	
% 	See Appendix~\ref{"proof-corolarry5.1"}
% \end{myproof}

%In order to use corollary \ref{"RCV-sup-control"} for a sequence  $V_{1:K}=(V_1,V_2,\dots,V_K)$, condition \eqref{"key-condition"}  must be checked.\,The following lemma establishes that the classical cross validation procedures verifies assumption 4.

% \begin{lemma}
% 	\label{"train-test-cond"}
% 	For leave-one-out,\,leave-$p$-out,\,and $K$-fold procedures,\,the training samples 
% 	$T_{1:K}$ and the validation samples $V_{1:K}$ satisfies assumption 4 i.e 
% 	\begin{equation*}
% 	\frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in T_j} }{n_{T}}= \frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in V_j} }{n_{V}}=\frac{1}{n} \quad \forall l \in \llbracket1,n\rrbracket.
% 	\end{equation*}
	
% \end{lemma}

% \begin{myproof}
% See appendix \ref{"proof-train-test-cond"}
% \end{myproof}
% \begin{remark*}
% 		For the $K$-fold  cross validation,\,the hypothesis $card(V_j)=n_{V}$ where $n_{V}$ is independent of $j$   only holds when $n$ is divisible by $K$. But even when $K$  does not divide $n$,\, one can obtain still similar results to those presented in this paper  by straightforward modifications of the proofs.
% 	\end{remark*}
	
% Combining corollary \ref{"RCV-sup-control"} and lemma \ref{"train-test-cond"} gives the following proposition.


% \begin{prop}\label{"key-proposition-CV"} 
% 	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables.\,For leave-one-out,\,leave-$p$-out,\,and $K$-fold procedures we have  
% 	\[\PP(Z-B(n_{V},\alpha)\geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right). \] 
% 	%
% %\quad \text{for } S_{1:K} \in \{T_{1:K},V_{1:K}\} \]
	
% 	where we recall that  $Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,S_{j})-\mathcal{R}(g) \rvert$.
% 	% and $n_S=card(S_1)$.	
% \end{prop}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_crossval.tex"
%%% End:


==> intermediate.tex <==
This section gathers generic concentration tools and technical intermediate results that are necessary to the proofs of our main results. %\,we introduce some intermediate results that will be used in this paper.

\subsection{Generic tools}
\label{sec:genericTools}


\,First,\,we recall the following McDiarmid's extension of Bernstein inequality (Theorem 3.8 in \cite{McDiarmid98conc}).
\begin{proposition}\label{"Bernstein-extension"}
	For a sequence of observations $(O_1,O_2,\dots,O_n) \in \mathcal{Z}^n$ and some fixed values $o_{1:l}=(o_1,o_2,\dots,o_l)$ and for some measurable function $f\,:\,\mathcal{Z}^n\rightarrow \rset$,\,let $Z=f(O_1,O_2,\dots,O_n)$ and define for $l \in \llbracket1,n\rrbracket$:
	\begin{enumerate}
		\item $f_{l}(o_1,o_2,\dots,o_l)=\mathbb{E}\left (Z \mid O_1=o_1,O_2=o_2,\dots,O_l=o_l\right),$ 
		\item $\Delta_l(o_1,o_2,\dots,o_{l-1},o_l)  =f_{l}(o_1,o_2,\dots,o_{l-1},o_l)-f_{l-1}(o_1,o_2\dots,o_{l-1}),$ (the positive deviations)
		\item $D:=\max _{l=1, \ldots, n} \sup _{o_{1}, \ldots, o_{i-1} \in \mathcal{X}} \sup _{o \in \mathcal{X}} \Delta_{l}\left(o_{1}, \ldots, o_{l-1}, o\right),$ (the maximum positive deviation)
		\item  $\sigma_{l}^2(o_{1:l-1})=\Var\left[ \Delta_l(O_1,O_2,\dots,O_{l-1},O' ) 
		\mid O_1=o_1, O_2=o_2 , \dots , O_{l-1}=o_{l-1} \right],$ where $O'$ is an independent copy of $O_1,$
            \item
              $\sigma^2=\sum_{l=1}^n \sup_{o_{1:l-1}\in
                \mathcal{X}^{l-1}} \sigma^2_l(o_{1:l-1})$ (the
              maximum sum of variances).
	\end{enumerate}
	Then we have
	\[ \PP(Z - \EE[Z] > t ) \le \exp{\left(\ffrac{-t^2}{2(\sigma^2 + Dt/3)}\right)}. \]
      \end{proposition}


We also recall Proposition 2.5.2 from \cite{vershynin_2018},\,which provides an upper bound for the expectation of sub-Gaussian random variables.
\begin{proposition}\label{"Expectation-UB-subgauss"}
Let $X$ be a real valued random variable and suppose that $$\PP(X\geq t)\leq C_1\exp{\left(-t^2/C_2^2\right)},$$ for some $C_1 , C_2 > 0$, then there exists a constant $M_2>0$ which depends only on $C_1$,\,such that
\[ \EE(X) \leq M_2 C_2.
\] 
\end{proposition}

      
%\vspace{10mm}
%In addition,\,to show the desired results,\,one need to make the following assumption :
%\begin{assumption}[mask property]\label{assum:mask-property}
%	The sequence of masks $S_1,S_2,\dots S_K$  verifies :
%	\begin{equation}\label{"card-condition"}
%	card(S_j)=n_S\quad \forall j \in \llbracket1,K\rrbracket
%	\end{equation}
%	for some $n_S \in \llbracket1,n\rrbracket$.\,Moreover :
%	\begin{equation}\label{"key-condition"}
%	\frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in S_j} }{n_S}=\frac{1}{n} \quad \forall l \in \llbracket1,n\rrbracket
%	\end{equation}
%\end{assumption}
%Later (lemma \ref{"train-test-cond"}),\,we will show that,\,when using the standard cross %validation procedures,\,the training and validation masks verifies this condition.\\
%First,\,let's use proposition \ref{"Bernstein-extension"} to prove the following lemma:
%
%\begin{lemma}
%	\label{"RCV-supp"}
%	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables, and $V_1,V_2,\dots V_K$ a sequence of masks that verifies assumption \ref{assum:mask-property} with size $n_V$.\,Moreover,\,suppose that assumption \ref{assum:hypo-class} and \ref{assum:cost-func} regarding the class $\mathcal{G}$ and $c$ hold.\,Define 
%	\begin{equation}\label{def:Z-CV}
%		Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,V_{j})-\mathcal{R}(g) \rvert,
%	\end{equation}
%	
% where $\Tilde{\mathcal{R}}_{\alpha}$ is defined by equation \ref{def:tilde-rcv}.\,Then the random variable $Z$  satisfies the Bernstein inequality	
%	
%	\[P\left(Z - E(Z) \geq t  \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).\]
%	
%\end{lemma}
%
%
%\begin{myproof}
% the reader is referred to appendix \ref{"lemma-RCV-supp-proof"}.
%	
%	
%\end{myproof}
%
%To obtain a probability bound of the estimate $Z$ via this lemma,\,one needs to control the term $E(Z)$.\,To do so, we will show a  result similar to lemma 14 in \cite{goix15}.
%\begin{lemma}
%	\label{"RCV-expectation"}
%        For any subsample $S\subset \{1,\ldots, n\}$ if size $n_S$ %mask $V$, and define
%	\[
%	Z'=\sup_{g \in \mathcal{G}} \bigg|\Tilde{\mathcal{R}}_{\alpha}(g,S)-\mathcal{R}(g)\bigg|.
%	\]
%	Then we have
%	\[
%	\EE(Z') \leq B(n_S,\alpha),
%	\]
%	with 
%\begin{equation}\label{"V-n-def"}
%  B(n_S,\alpha)= \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n_S}}
%%  {\color{red} + \frac{M_1  \vapnikG}{\alpha n_S}}
%\end{equation}  
%for some constant $M>0$.
%\end{lemma}
%
%\begin{myproof}
%	
%	See appendix \ref{"proof-RCv-expectation"}
%\end{myproof}
%
%
%Combining lemma \ref{"RCV-supp"} and lemma \ref{"RCV-expectation"} allows to deduce the following corollary. 
%
%\begin{corollary}
%	\label{"RCV-sup-control"}
%	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables, and $V_1,V_2,\dots V_K$ a sequence of masks satisfying assumption \ref{assum:mask-property} .\, In addition suppose that assumption \ref{assum:hypo-class} and \ref{assum:cost-func} hold.\,then we have
%	\[P\left(Z - B(n_V,\alpha) \geq t \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right),\]
%	where $Z$ and $B$ are defined by equations \ref{def:Z-CV} and \ref{"V-n-def"} respectively.
%	
%\end{corollary}

%\begin{myproof} The idea is to show that $E(Z) \leq B(n_S,\alpha)$ and to conclude by using Lemma \eqref{"RCV-supp"}.\,To do so,\,notice that for 2 different masks  $V_{j}$ and $V_{j'}$ we have $\mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_j)- \mathcal{R}_{\alpha}(g)\bigg|\right]= \mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_{j'})- \mathcal{R}_{\alpha}(g)\bigg|\right]$ since all observations are i.i.d and the  vectors $V_j$'s have all the same length. Thus it follows that
%	\[\mathbb{E}\left[\ffrac{1}{K}\sum_{j=1}^K\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_j)- \mathcal{R}_{\alpha}(g)\bigg|\right]=
%	\mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_1)- \mathcal{R}_{\alpha}(g)\bigg|\right].\]
%	
%	
%	Now using Lemma  \ref{"RCV-expectation"} one obtains 
%	\[\underbrace{\mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_1)- \mathcal{R}_{\alpha}(g)\bigg|\right]}_{\mathbb{E}(Z) } \leq \underbrace{\ffrac{M\sqrt{\mathcal{V}_{\mathcal{G}}}}{\sqrt{n_{S}\alpha}}}_{B(n_{S},\alpha)}.\]
%	
%	Combining this with lemma \ref{"RCV-supp"} yields the desired result.  
%%	\[\PP(Z-B(n_{S},\alpha)\geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right)\]
%\end{myproof}


%In order to use corollary \ref{"RCV-sup-control"} for a sequence  $V_{1:K}=(V_1,V_2,\dots,V_K)$, condition \eqref{"key-condition"}  must be checked.\,In the following lemma, we show that the classical cross validation procedures verifies assumption 4.
%
%\begin{lemma}
%	\label{"train-test-cond"}
%	For leave-one-out,\,leave-$p$-out,\,and $K$-fold procedures,\,the training samples 
%	$T_{1:K}$ and the validation samples $V_{1:K}$ satisfies assumption 4 i.e 
%	\begin{equation*}
%	\frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in T_j} }{n_{T}}= \frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in V_j} }{n_{V}}=\frac{1}{n} \quad \forall l \in \llbracket1,n\rrbracket.
%	\end{equation*}
%	
%\end{lemma}
%
%\begin{myproof}
%%	
%	Since the leave-one-out can be seen as a special case of $K$-fold, with $K=n$ it suffices to treat only the case of leave-$p$-out and $K$-fold .
%	
%	\paragraph{$K$-Fold.} For this procedure,\,the validation "masks" verifies the following property
%	\begin{equation}\label{"loo-k-fold-prop"}
%	\bigcup\limits_{j=1}^K V_j=\llbracket1,n\rrbracket \: and \: V_j\bigcap V_k=\varnothing\:, \:\forall j\neq k \in \llbracket1,K\rrbracket.
%	\end{equation}
%	
%	Under the hypothesis that $card(V_j)=n_{V}$  for all the validation sets, \eqref{"loo-k-fold-prop"} implies\,that
%	\begin{equation}
%	\label{"K-fold-equation"}
%	n=\sum_{j=1}^{K}card(V_j)=Kn_{V}. 
%	\end{equation}
%	
%	
%	Furthermore,\,under \eqref{"loo-k-fold-prop"},\,an index $l\in \llbracket 1,n \rrbracket$ belongs to a unique validation test $V_j'$ and to all the train sets $T_j=V_j^c$ with $j\neq j'$.\,Hence,\,we have
%	
%	\begin{equation*}
%	\begin{cases}
%	\sum_{j=1}^{K}\indic{l \in T_j} = K-1, \\
%	\sum_{j=1}^{K}\indic{l \in V_j} = 1.
%	\end{cases}  
%	\end{equation*}
%	Using \eqref{"K-fold-equation"} and the fact that $n_{T}=n-n_{V}=(K-1)n_{V}$ yields the desired result.
%%	
%%	\begin{equation*}
%%	\begin{cases}
%%	\ffrac{1}{Kn_{T}}\sum_{j=1}^{K}\indic{l \in T_j} = 1/n \\[10pt]
%%	\ffrac{1}{Kn_{V}}\sum_{j=1}^{K}\indic{l \in V_j} = 1/n,
%%	\end{cases}  
%%	\end{equation*}
%%	
%%	which is the desired result.
%	
%	\paragraph{Leave-$p$-out.}
%	In the leave-$p$-out procedure,\,the validation sets are all the subsamples of $\DD_n$ with $card(V_j)=p$,\,thus we have\,$K=\binom{n}{p}$. On the other hand,\,an index $l\in \llbracket 1,n \rrbracket$ belongs to $\binom{n-1}{p-1}$ validation sets.\,In fact, creating a $V_j$ such as $l \in V_j$ is equivalent to first picking $l$  and then choosing $m-1$  element from $\llbracket1,n\rrbracket \setminus \{l\}$.
%	Hence we have
%	
%	\begin{equation*}
%	\sum_{j=1}^{K}\indic{l \in V_j} = \binom{n-1}{p-1} \: \, , \: \forall l \in \llbracket1,n\rrbracket.
%	\end{equation*}
%	Recall that $n\binom{n-1}{p-1}=p\binom{n}{p}$ which yields 
%	\[\ffrac{1}{Kn_{V}}\sum_{j=1}^{K}\indic{l \in V_j}= \ffrac{1}{p\binom{n}{p}}\sum_{j=1}^{K}\indic{l \in V_j}= 1/n. \]
%	
%	Similar arguments can be used for the sequence $T_{1:K}$,\,and the proof is complete.
%	
%	\begin{remark*}
%		For the $K$-fold  cross validation,\,the hypothesis $card(V_j)=n_{V}$ where $n_{V}$ is independent of $j$   only holds when $n$ is divisible by $K$. But even when $K$  does not divide $n$,\, one can obtain still similar results to those presented in this paper  by straightforward modifications of the proofs.
%	\end{remark*}
%\end{myproof}

%Combining corollary \ref{"RCV-sup-control"} and lemma \ref{"train-test-cond"} gives the following proposition.
%
%
%\begin{prop}\label{"key-proposition-CV"} 
%	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables.\,For leave-one-out,\,leave-$p$-out,\,and $K$-fold procedures we have  
%	\[\PP(Z-B(n_{V},\alpha)\geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right). \] 
%	%
%%\quad \text{for } S_{1:K} \in \{T_{1:K},V_{1:K}\} \]
%	
%	where we recall that  $Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,S_{j})-\mathcal{R}(g) \rvert$.
%	% and $n_S=card(S_1)$.	
%\end{prop}

\subsection{Technical results}\label{sec:technicalResults}

\begin{lemma}\label{"RCV-ge-RN"}
Let $\Psi_{\alpha}$ be the ERM rule on the tail region of level $1-\alpha$ defined in (\ref{"g_alpha_j_def"}). Given a dataset	$\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ and a sequence of mask $V_{1:K}$ it holds that
\[   
\widehat{ \mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),S_n) \leq  \widehat{\mathcal{R}}_{CV,\alpha}(\Psi_{\alpha},V_{1:K}).
\]
In other words the \CV risk estimate of the ERM rule cannot be less than the empirical risk evaluated on the full dataset. 
\end{lemma}


\begin{proof}
The argument for $\alpha\neq 1$ is the same as the one for
 $\alpha=1$ (standard ERM) which may be found in \cite{kearns1999algorithmic}. We reproduce
  it for the sake of completeness. By definition of
  $\Psi_{\alpha}(S_n)$,\,one has

\begin{equation*}
  \forall j \in \llbracket 1,n \rrbracket \:,\: \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),S_n) \geq \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),S_n).
\end{equation*}

Since $\widehat{\mathcal{R}}_{\alpha}(g,S_n)= \ffrac{1}{n}\left( n_{V}\widehat{\mathcal{R}}_{\alpha}(g,V_j)+n_{T}\widehat{\mathcal{R}}_{\alpha}(g,T_j) \right)$, for $g\in \mathcal{G}$.\,It follows that
\begin{align*}
	\ffrac{1}{n}\left( n_{V}\underbrace{\widehat{\mathcal{R}}_{\alpha}(\Psi_\alpha(T_j),V_j)}_{\text{validation error}}+n_{T}\underbrace{\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),T_j)}_{\text{training error}}  \right) \geq \ffrac{1}{n}\big( n_{V}\widehat{\mathcal{R}}_{\alpha}(&\Psi_{\alpha}(S_n),V_j)\\& +  n_{T}\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),T_j) \big).
\end{align*}


Since $\Psi_{\alpha}(T_j)$ minimizes the training error on the $j$'th train set $T_j$, in particular we have $$\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),T_j) \geq  \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),T_j),$$ hence %it follows that
\begin{equation}\label{ineq:cv-er-base}
	\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),V_j) \leq  \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),V_j)\:,\:\forall j \in \llbracket 1 , K \rrbracket.
\end{equation}

In addition the average empirical risk of $\Psi_\alpha(S_n)$ is equal to its empirical risk on the full dataset, indeed
\begin{align*}
	\ffrac{1}{K}\bigg(\sum_{j=1}^{K}\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),V_j)\bigg)&=\ffrac{1}{Kn_{V}}\bigg(\sum_{j=1}^{K}\sum_{i\in V_j} c\big(\Psi_{\alpha}(S_n),O_i)\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor\big)}\rVert }\bigg)\\
	&=\ffrac{1}{Kn_{V}}\bigg(\sum_{j=1}^{K}\sum_{i=1}^{n}c\big(\Psi_{\alpha}(S_n),O_i\big)\un{i \in V_j}\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor)}\rVert }\bigg)\\
	&=\ffrac{1}{Kn_{V}}\bigg(\sum_{i=1}^{n}c\big(\Psi_{\alpha}(S_n),O_i\big)\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor)}\rVert }\bigg)\sum_{j=1}^{K}\un{i \in V_j}\\
	(\text{By lemma }\ref{"train-test-cond"})&=\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n)).
\end{align*}

Thus \,by averaging inequality \ref{ineq:cv-er-base}, we get
\[   
\widehat{ \mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),S_n) \leq  \widehat{\mathcal{R}}_{CV,\alpha}(\Psi_{\alpha},V_{1 : K}).
\]
\end{proof}
The following lemma is used in the proof of our second main result concerning \lpo risk estimation, see inequality~(\ref{eq:keyTheorem2fromLemma}). It is a generalization of  Markov inequality that is particularly useful for  cross-validation estimates. Our proof shares similarities with the proof of Theorem 4.1 in~\cite{kearns1999algorithmic} formulated under general algorithmic stability assumptions. 
\begin{lemma}\label{"RCV-markov"}
In the setting of Theorem \ref{theo:main-sanity-rare}, we have 
\begin{align*}
	\PP(\rcvEx(\Psi_{\alpha},V_{1 : K}) - \mathcal{R}_{CV,\alpha}(\Psi_{\alpha},V_{1 : K})  \geq &t ) \leq \\
	&\ffrac{\EE(\DevExt+\BiasCV+\abs{ \hat\risk_\alpha(\Psi_{\alpha}(S_n),S_n) - \risk_\alpha(\Psi_{\alpha}(S_n)) })}{t},
\end{align*}

where  $\BiasCV$ (resp $\DevExt$) is defined by equation \ref{"bias_CV"} (resp \ref{"dev_ext"}).
\end{lemma}

\begin{proof}
Set 
$\rcvEx=\rcvEx(\Psi_{\alpha},V_{1 : K})$, $\mathcal{R}_{CV,\alpha}=\mathcal{R}_{CV,\alpha}(\Psi_{\alpha},V_{1 : K})$ , $  \hat\risk_\alpha=\hat\risk_\alpha(\Psi_{\alpha}(S_n),S_n)$, $ \risk_\alpha=\risk_\alpha(\Psi_{\alpha}(S_n))$.\\
 For any integrable real valued random variable $W$, and any $t>0$ write  
  $$\EE[W]= \PP[W\ge t]\EE[W \,|\, W\ge t] + \EE[W \un{W<t}].$$ Reorganising, we obtain the following generalized Markov inequality, 
  \[
    \PP[W>t] = \frac{\EE[W] - \EE[W \un{W<t}]}{\EE[W \,|\, W\ge t]}
    \le \frac{\EE(W) - \EE(W \un{W<t})}{t}. 
  \]
  Letting $W = \rcvEx-\mathcal{R}_{CV,\alpha}$ we obtain
%     \begin{equation*}
%      \begin{split}
% \EE(\rcvEx-\mathcal{R}_{CV,\alpha})=\PP(\rcvEx&-\mathcal{R}_{CV,\alpha}\geq t)\EE(\rcvEx-\mathcal{R}_{CV,\alpha} \mid \rcvEx-\mathcal{R}_{CV,\alpha} \geq t)\\&+\EE\left[(\rcvEx-\mathcal{R}_{CV,\alpha}) \indic{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right].
% \end{split}
% \end{equation*} 
% Thus one obtains 
\begin{equation}
\label{"exp-CV-one"}
\PP(\rcvEx-\mathcal{R}_{CV,\alpha}\geq t)= \frac{\EE(\rcvEx-\mathcal{R}_{CV,\alpha})-\EE\left[(\rcvEx-\mathcal{R}_{CV,\alpha}) \un{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right]}{t}.
\end{equation} 


Using the fact that $\EE(\tilde{\mathcal{R}}_{CV,\alpha}-\risk_{CV,\alpha})=0$ and that $\DevExt=\abs{\rcvEx-\tilde{\mathcal{R}}_{CV,\alpha}}$, one gets
\begin{align}
\EE(\rcvEx-\mathcal{R}_{CV,\alpha})&=\EE(\rcvEx-\tilde{\mathcal{R}}_{CV,\alpha}) \nonumber \\ &\leq \EE(\DevExt).
\label{"exp-CV-two"}
\end{align} 
Now using lemma  \ref{"RCV-ge-RN"} write

\begin{align}
\EE\left[(\mathcal{R}_{CV,\alpha}-\rcvEx) \ind_{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right] &\leq \EE\left[(\mathcal{R}_{CV,\alpha}-\widehat\risk_\alpha) \ind_{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right] \nonumber \\ & \leq \EE\left[\abs{\mathcal{R}_{CV,\alpha}-\widehat\risk_\alpha} \ind_{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right]  \nonumber \\ & 
\leq  \EE\left[\abs{\mathcal{R}_{CV,\alpha}-\widehat\risk_\alpha} \right] \nonumber \\ &
\leq \EE\left[\abs{\mathcal{R}_{CV,\alpha}-\risk_\alpha} \right]+ \EE\left[\abs{\risk_\alpha-\widehat\risk_\alpha} \right] \nonumber \\
&=\EE\left[\BiasCV \right]+ \EE\left[\abs{\risk_\alpha-\widehat\risk_\alpha} \right].
\label{"exp-CV-three"}
\end{align}

The last line follows from the definition of $\BiasCV$ in (\ref{"bias_CV"}). Combining inequality \eqref{"exp-CV-one"} with equations \eqref{"exp-CV-two"} and \eqref{"exp-CV-three"} yields
	\[\PP(\rcvEx-\mathcal{R}_{CV,\alpha} \geq t ) \leq \ffrac{\EE(\DevExt+\BiasCV+\abs{\hat\risk_\alpha- \risk_{\alpha}})}{t}, \]
which concludes the proof.
\end{proof}

To conclude this section, we extend Theorem~10 in~\cite{goix15} bounding the supremum deviations of the empirical measure on low probability regions, to handle the case of any cost function $c$ absolutely bounded by one.
\begin{lemma}\label{lemma:inv-goix}
Recall the definitions of the risk $\risk_\alpha$ and its empirical version $\ER_\alpha$ given in Section~\ref{sec:framework} and introduce the (random) supremum deviations 
		\[Z'=\sup_{g \in \mathcal{G}}\lvert \widehat{\mathcal{R}}_{\alpha}(g,S_n)-\mathcal{R}_\alpha(g) \rvert.\]
If $\mathcal{G}$ is a family of classifiers with finite VC-dimension and $c$ a bounded cost function with $\sup_{g,o}|c(g,o)|\le 1$, then,  the following Bernstein-type  inequality holds, 
	\[ \PP(Z'-Q(n,\alpha) \geq t)\leq 3\exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right), \]
	where $Q(n,\alpha)=B(n,\alpha)+\ffrac{1}{n\alpha}$ and $B$ is defined by
        %
        % equation \ref{"V-n-def"}.
\begin{equation}\label{"V-n-def"}
  B(n,\alpha) = \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n}} %  {\color{red} + \frac{M_1  \vapnikG}{\alpha n_S}},
\end{equation}  
and $M$ is a universal constant. 
        
\end{lemma}

\begin{proof}
	Write $Z' \leq Z_1 +Z_2$ with :
	\[Z_1=\sup_{g \in \mathcal{G}}\lvert \widehat{\mathcal{R}}_{\alpha}(g,S_n)-\Tilde{\mathcal{R}}_{\alpha}(g,S_n) \rvert,\]
	\[ Z_2=\sup_{g \in \mathcal{G}}\lvert\Tilde{\mathcal{R}}_{\alpha}(g,S_n)-\mathcal{R}_{\alpha}(g)\rvert.\]
Concerning $Z_2$, applying Corollary \ref{"RCV-sup-control"} with $K=1$ , $V_1=S_n$, $\mathcal{A}=(\lVert X \rVert \geq t_\alpha)$, yields
		\begin{equation}\label{ineq:Z-1-UB}
	\PP(Z_2 - B(n,\alpha) \geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).
	\end{equation}
We now focus on $Z_1$. Define 
$$u_{i}=\left|\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor)}\rVert}
-\un{\lVert X_{i} \rVert \geq t_\alpha}\right|$$ 
and notice that $ Z_1\leq \ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i}$. It is known (see for instance the bound for the term $A$ in \cite{jalalzai2018binary}, page 12) that 
\begin{equation*}
\ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i}\leq  \frac{1}{\alpha}\left|\frac{1}{n}\sum_{i= 1}^n \un{\lVert X\rVert \geq t_\alpha}-\alpha\right| + \frac{1}{n\alpha}. 
\end{equation*}
Now,  by noticing that $\Var(\indic{\lVert X\rVert \geq t_\alpha}) \le \alpha$ and using Bernstein's inequality, we get
\begin{align*}
\PP\left(\bigg|\frac{1}{n}\sum_{i= 1}^n \indic{\lVert X\rVert \geq t_\alpha}-\alpha \bigg|\geq t\right)&\leq 2\exp\left(\ffrac{-n t^2}{2(\alpha+t/3)}\right)\\&\leq 2\exp\left(\ffrac{-n t^2}{2(4\alpha+t/3)}\right).
\end{align*}
Finally,\,dividing by $\alpha$, we get 
% and noticing that  $P(\abs{X}\geq t) \leq P(X\geq t)+ P(-X\geq t) $ leads to 
\begin{align*}
\PP(\frac{1}{\alpha}&\bigg|\sum_{i= 1}^n \frac{1}{n}\indic{\lVert X\rVert \geq t_\alpha}-\alpha\bigg| \geq t)\leq 2\exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).
\end{align*}
Therefore we finally obtain
\begin{equation}\label{bound:z1}
\PP\left(  \ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i} - 1/n\alpha  \geq t \right) \leq  2\exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).
\end{equation}
The result follows using $Z' \leq Z_1 + Z_2$ and $ Z_1\leq \ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i}$.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_crossval.tex"
%%% End:

